Rational spectral filters with optimal convergence rate

In recent years, contour-based eigensolvers have emerged as a standard approach for the solution of large and sparse eigenvalue problems. Building upon recent performance improvements through non-linear least square optimization of so-called rational filters, we introduce a systematic method to design these filters by minimizing the worst-case convergence ratio and eliminate the parametric dependence on weight functions. Further, we provide an efficient way to deal with the box-constraints which play a central role for the use of iterative linear solvers in contour-based eigensolvers. Indeed, these parameter-free filters consistently minimize the number of iterations and the number of FLOPs to reach convergence in the eigensolver. As a byproduct, our rational filters allow for a simple solution to load balancing when the solution of an interior eigenproblem is approached by the slicing of the sought after spectral interval.

==> figures/alg_slise.tex <==
% !TeX spellcheck = en_US
\begin{algorithm}[t]
 \caption{(\SLISE{} minimization through \BFGS{})}
 \label{alg:slise}
 \algoheader{An existing rational filter $\ratcp{r}{\beta^{(0)},z^{(0)}}$,
 for
  some $\beta^{(0)} \in \C^m$, $z^{(0)} \in (\C \setminus \R)^m$, $m \in 
  \N$,
  and\\a
  weight function $\wgtf$.}{A new rational filter
  $\ratcp{r}{\beta',z'}$, where $(\beta', z')$ is a minimizer of the
  objective function $f_{\wgtf}$ and $\beta' \in \C^m, z' \in (\C
   \setminus \R)^m$.}
 \begin{algorithmic}[1]
  \Function{\SLISEtext{}}{$\beta^{(0)},z^{(0)},\wgtf$}
  \State
  %\st{$\beta',z'\gets$ Apply \BFGS{} minimization algorithm
  %to $f_{\wgtf}$ with starting point
  %$(\beta^{(0)},z^{(0)})$.}
  \State $\beta',z'\gets$ BFGS$(f_{\wgtf}, \nabla f_{\wgtf},
  \beta^{(0)},z^{(0)})$ \cmt{}{Does a function that calls another function
    makes even sense?}
  \State %\st{\Return $(\beta',z')$}
  \State \Return $\ratcp{r}{\beta',z'}$ to be consistent with the
  definition of Eq. (14). $w_G$ is a function of $r$ not of $(\beta, z)$. 
  \EndFunction
 \end{algorithmic}
\end{algorithm}


==> figures/alg_wwcr.tex <==
\begin{algorithm} [t] %[h!t]
 \caption{(Weight function \WCR{} (\WWCR{}))}
 \label{alg:weight_worst}
 \algoheader{A weight function $\wgtf$, a rational filter
  $\ratcp{r}{\beta,z}$ whose robustness shall be improved, and a gap
  parameter $G \in (0,1)$, while $\beta \in \C^m$, $z \in (\C
   \setminus \R)^m$, $m \in \N$.}{The $w_G$ value of the 
   \SLISE{} filter that may be obtained from the inputs.}
 \begin{algorithmic}[1]
  \Function{\WWCRtext{}}{$\wgtf,G,\beta,z$}
  \State $\beta',z'\gets$ \Call{\SLISEtext{}}{$\beta,z,\wgtf$}
  \State $a\gets$ \Call{$w_G$}{$\ratcp{r}{\beta',z'}$}
  \Comment{Robustness of \SLISE{} filter  $\ratcp{r}{\beta',z'}$, as per 
  \eqref{eqn:worst}}
  \State \Return $a$
  \EndFunction
 \end{algorithmic}
\end{algorithm}

==> figures/filters_shifting.tex <==
\begin{figure}
	\centering			
	\tikzsetnextfilename{filters_shifting}
	\begin{tikzpicture}
	\begin{axis}[
	xmin=0.9,
	xmax=1.1,
	xtick={0.9,0.974679434,1,1.05,1.1},
	xticklabels={$0.9$,$\sqrt{G}=0.9747$,$1.0$,$1.05$,$1.1$},
	ymode=log,
	ytick={0.000000001,0.000001,0.001,1},
	yticklabels={$10^{-9}$,$10^{-6}$,$10^{-3}$,$10^{0}$},
	%legend pos=south west,
	xlabel={$\abs{x}$}, ylabel={Absolute Filter Value (log)},
	width=0.9\textwidth,
	height=0.24\textheight,
	%legend pos=south west,
	legend style={at={(0.5,1.1)}, anchor=south,legend columns=-1},
	]	
	\addplot[color=SLISEC3, thick] table[x index={0},y 
	expr=abs(\thisrowno{1})] {figures/wcr_4_95_accuracy.dat};
	\addplot[color=SLISEC, thick] table[x index={0},y 
	expr=abs(\thisrowno{2})] {figures/wcr_4_95_accuracy.dat};
	
	\addlegendentry{Shifted, \WCR{}-reduced, $G=0.95$}
	\addlegendentry{Unshifted, \WCR{}-reduced, $G=\sqrt{0.95}$}
	\end{axis}
	\end{tikzpicture}
	\caption{Logarithmic plot to illustrate shifting of rational filters.
	The unshifted filter is a solution of the previous minimization 
	problem in \eqref{eqn:minweight} for $G=\sqrt{0.95}$,
	while the shifted filter solves the new minimization problem as of
	\eqref{eqn:newwcr} for $G=0.95$.
	}
	\label{fig:filters_shifting}
\end{figure}
